DeepZensols: Deep Natural Language Processing Framework

Reproducing results in publications by distributing publicly available source code is becoming ever more popular. Given the difficulty of reproducing machine learning (ML) experiments, there have been significant efforts in reducing the variance of these results. As in any science, the ability to consistently reproduce results effectively strengthens the underlying hypothesis of the work, and thus, should be regarded as important as the novel aspect of the research itself. The contribution of this work is a framework that is able to reproduce consistent results and provides a means of easily creating, training, and evaluating natural language processing (NLP) deep learning (DL) models.

==> makefile <==
# Paul Landes - 6/20/2018
# export version makefile
# https://github.com/plandes/zenbuild

# binaries
TEX_LATEX_CMD =	pdflatex
BIBTEX=		bibtex
BIBER=		biber
BIB_FILE=	$(wildcard *.bib)

# files
TEX=		DeepZensols
TEX_LATEX_FILE=	$(TEX).tex
TEX_PDF_FILE=	$(TEX).pdf
TEX_FINAL_RUNS =3

all:		pdf

.PHONY:		info
info:
		@echo "name: $(TEX)"
		@echo "tex: $(TEX_LATEX_FILE)"
		@echo "pdf: $(TEX_PDF_FILE)"
		@echo "bib-file: $(BIB_FILE)"

.PHONY:		pdf
pdf:		$(TEX_PDF_FILE)

$(TEX_PDF_FILE):	$(TEX_LATEX_FILE)
		$(TEX_LATEX_CMD) $(TEX).tex
		if [ -f "$(BIB_FILE)" ] ; then \
			if [ -f zenbiber ] ; then \
				$(BIBER) $(TEX) ; \
			else \
				$(BIBTEX) $(TEX) ; \
			fi \
		fi
		for i in `seq $(TEX_FINAL_RUNS)` ; do \
			$(TEX_LATEX_CMD) $(TEX).tex ; \
		done

clean:
		rm -f *.pdf *.out *.aux *.log *.bbl *.bcf *.blg \
			*.upa *.upb *.xml zenbiber

